AnyMoLe: Any Character Motion In-betweening Leveraging Video Diffusion Models

Despite recent advancements in learning-based motion in-betweening, a key limitation has been overlooked: the requirement for character-specific datasets. In this work, we introduce AnyMoLe, a novel method that addresses this limitation by leveraging video diffusion models to generate motion in-between frames for arbitrary characters without external data. Our approach employs a two-stage frame generation process to enhance contextual understanding. Furthermore, to bridge the domain gap between real-world and rendered character animations, we introduce ICAdapt, a fine-tuning technique for video diffusion models. Additionally, we propose a ``motion-video mimicking'' optimization technique, enabling seamless motion generation for characters with arbitrary joint structures using 2D and 3D-aware features. AnyMoLe significantly reduces data dependency while generating smooth and realistic transitions, making it applicable to a wide range of motion in-betweening tasks.

==> fig_tex/x_generated1.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.95\linewidth]{fig/gen2.png}
\caption{Visual results of generated in-between motion frames.}
\label{fig:x_gen1}
\end{figure*}

==> fig_tex/x_generated2.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.95\linewidth]{fig/gen1.png}
\caption{Visual results of generated in-between motion frames.}
\label{fig:x_gen2}
\end{figure*}

==> fig_tex/x_jointestimator.tex <==
\begin{figure*}[t]
\centering
\vspace{3mm}
\includegraphics[width=\linewidth]{fig/scenespecific.png}
\caption{Architecture of scene specific joint estimator.}
\label{fig:x_joint}
\end{figure*}

==> fig_tex/x_video1.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{fig/ablation_add3.png}
\vspace{-6mm}
\caption{Additional results of the ablation study on video generation.}
\label{fig:x_video1}
\end{figure*}

==> fig_tex/x_video2.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{fig/ablation_add.png}
\vspace{-6mm}
\caption{Additional results of the ablation study on video generation.}
\label{fig:x_video2}
\end{figure*}
